Deep Recurrent Q-learning for Energy-constrained Coverage with a Mobile Robot

In this paper, we study the problem of coverage of an environment with an energy-constrained robot in the presence of multiple charging stations. As the robot's on-board power supply is limited, it might not have enough energy to cover all the points in the environment with a single charge. Instead, it will need to stop at one or more charging stations to recharge its battery intermittently. The robot cannot violate the energy constraint, i.e., visit a location with negative available energy. To solve this problem, we propose a deep Q-learning framework that produces a policy to maximize the coverage and minimize the budget violations. Our proposed framework also leverages the memory of a recurrent neural network (RNN) to better suit this multi-objective optimization problem. We have tested the presented framework within a 16 x 16 grid environment having charging stations and various obstacle configurations. Results show that our proposed method finds feasible solutions and outperforms a comparable existing technique.

==> illust.tex <==



\begin{tikzpicture}[scale=0.7]
\draw[step=1cm,gray,very thin] (-2,-2) grid (6,6);
\filldraw[fill=black!40!white, draw=black] (0,0) rectangle (2,2);
\filldraw[fill=black!40!white, draw=black] (2,5) rectangle (6,6);

\filldraw[fill=green!70!white, draw=black] (-2,-2) rectangle (-1,-1);
\node [quadcopter top,fill=white,draw=black,minimum width=1cm,rotate=20,scale=0.5] at (-1.5,-1.5) {}; 
\filldraw[fill=green!70!white, draw=black] (4,1) rectangle (5,2);
\filldraw[fill=green!70!white, draw=black] (1,5) rectangle (2,6);

\draw[red,thick,dashed,->] (4.5,1.5) -- (4.5,2.5);
\draw[red,thick,dashed,->] (4.5,1.5) -- (4.5,0.5);
%\draw[red,thick,dashed,->] (4.5,1.5) -- (3.5,2.5);
\draw[red,thick,dashed,->] (4.5,1.5) -- (3.5,1.5);
%\draw[red,thick,dashed,->] (4.5,1.5) -- (3.5,0.5);
%\draw[red,thick,dashed,->] (4.5,1.5) -- (5.5,2.5);
\draw[red,thick,dashed,->] (4.5,1.5) -- (5.5,1.5);
%\draw[red,thick,dashed,->] (4.5,1.5) -- (5.5,0.5);
\end{tikzpicture}

==> source files/NN_model.tex <==



\def\ConvColor{rgb:yellow,5;red,1.5;white,5}
\def\ConvReluColor{rgb:yellow,5;red,15;white,5}
\def\PoolColor{rgb:red,1;black,0.3}
\def\DcnvColor{rgb:blue,5;green,2.5;white,5}
\def\SoftmaxColor{rgb:magenta,5;black,7}
\def\SumColor{rgb:blue,5;green,15}
\def\poolsep{1}

\tikzset{
connector/.style={
     -latex,
     font=\scriptsize
    },
rectangle connector/.style={
        connector,
        to path={(\tikztostart) -- ++(#1,0cm) \tikztonodes |- (\tikztotarget) },
        pos=0.5
    },
    rectangle connector/.default=-2cm,
    straight connector/.style={
        connector,
        to path=--(\tikztotarget) \tikztonodes
    }
    }
\tikzset{every loop/.style={min distance=20mm%,in=0,out=120,looseness=50
}}

\begin{tikzpicture}
\tikzstyle{connection}=[thick,every node/.style={sloped,allow upside down},draw=\edgecolor,opacity=0.6]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Draw Layer Blocks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\draw[red] (-11,-5,0) rectangle (-3,1,0);
% conv1_1,conv1_2,%pool1
\pic[shift={(0,0,0)}] at (0,0,0) {RightBandedBox={name=cr1,caption=Conv 1,%
        fill=\ConvColor,bandfill=\ConvReluColor,%
        height=10,width={1},depth=10}};
% conv2_1,conv2_2,pool2
\pic[shift={(1,0,0)}] at (cr1-east) {RightBandedBox={name=cr2,caption=Conv 2,%
        fill=\ConvColor,bandfill=\ConvReluColor,%
        height=10,width={1},depth=10}};

% conv3_1,conv3_2,pool3
% \pic[shift={(1,0,0)}] at (cr2-east) {RightBandedBox={name=cr3,caption=Conv 3,%
%         xlabel={{"l","l","l"}},zlabel=,fill=\ConvColor,bandfill=\ConvReluColor,%
%         height=10,width={1,1,1},depth=10}};


%%State Input
%% action input
\pic[shift={(-2,0,0)}] at (cr1-west) {Box={name=states,caption=State Input,%
xlabel={{"","dummy"}},fill=,opacity=0.01,height=5,width=3,depth=5}};

% conv4_1,conv4_2,conv4_3,pool4
% \pic[shift={(1,0,0)}] at (p3-east) {RightBandedBox={name=cr4,%
%         xlabel={{"512","512","512"}},zlabel=I/8,fill=\ConvColor,bandfill=\ConvReluColor,%
%         height=10,width={1,1,1},depth=10}};
% \pic[shift={(\poolsep,0,0)}] at (cr4-east) {Box={name=p4,%
%         fill=\PoolColor,opacity=0.5,height=8,width=1,depth=8}};
% % conv5_1,conv5_2,conv5_3,pool5
% \pic[shift={(1,0,0)}] at (p4-east) {RightBandedBox={name=cr5,%
%         xlabel={{"512","512","512"}},fill=\ConvColor,bandfill=\ConvReluColor,%
%         height=8,width={1,1,1},depth=8}};
%% fc8 -> cr8 (score32)


%% first linear layer   
% \pic[shift={(1,-3,0)}] at (cr1-south) {Box={name=acfc,caption=Linear,%
% xlabel={{"$1$","dummy"}},zlabel={$\qquad 32$},fill=\SumColor,opacity=0.3,height=2,width=2,depth=15}};

%% action input
% \pic[shift={(-1,-3,0)}] at (cr1-south) {Box={name=acts,caption=Action Input,%
% xlabel={{"","dummy"}},zlabel=$\quad a_t$,fill=,opacity=0.01,height=5,width=3,depth=5}};

        
%% LSTM layer    
\pic[shift={(2.5,0,0)}] at (cr2-east) {Box={name=lstm,caption=LSTM,%
        %xlabel={{"$1$","dummy"}},zlabel={$128$},
        fill=,opacity=0.5,height=5,width={7},depth=3,fill=\SoftmaxColor}};
        
\node[circle, draw=red] (anch) [left=of lstm-west] {$+$};

\node[draw=none] (budget) [below=of anch,yshift=-0.2cm] {Budget};
        
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\skipshift{6.5}
%%Joining with previous streams (fcn-16)
%% score16
% \pic[shift={(0,0,3+\skipshift)}] at (cr5-anchor) {Box={name=score8,%
%         xlabel={{"K","dummy"}},fill=\ConvColor,height=10,width=2,depth=10,zlabel=I/8}};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Joining with previous streams (fcn-8)
%% score8
% \pic[shift={(0,5,8+\skipshift)}] at (cr4-east) {Box={name=score4,%
%         xlabel={{"K","dummy"}},fill=\ConvColor,height=10,width=2,depth=10,zlabel=I/4}};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Joining with previous streams (fcn-4)
%% score4
% \pic[shift={(0,8,13+\skipshift)}] at (cr3-east) {Box={name=score2,%
%         xlabel={{"K","dummy"}},fill=\ConvColor,height=10,width=2,depth=10,zlabel=I/2}}; 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Joining with previous streams (fcn-2)
%% score2
% \pic[shift={(0,8,22+\skipshift)}] at (p2-east) {Box={name=score,%
%         xlabel={{"K","dummy"}},fill=\ConvColor,height=10,width=2,depth=10,zlabel=I}};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Linear 2 (after LSTM)
\pic[shift={(1.5,0,0)}] at (lstm-east) {Box={name=lin2,caption=Linear, %xlabel={{"$1$","dummy"}},
zlabel={$\qquad 128$},
fill=\SumColor,opacity=0.3,height=2,width=2,depth=15}};

%% Output layer
\pic[shift={(1.5,0,0)}] at (lin2-east) {Box={name=output,caption=Output,%
        xlabel={{"$\vert\mathcal{A}\vert$","dummy"}},fill=\DcnvColor,height=10,width=1,depth=0,zlabel=}};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Draw connections
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw [connection]  (states-east)      -- node {\midarrow} (cr1-west);

\draw [connection]  (cr1-east)      -- node {\midarrow} (cr2-west);
% \draw [connection]  (cr2-east)      -- node {\midarrow} (cr3-west);
\draw [connection]  (cr2-east)    -- node {\midarrow} (anch);
\draw [connection]  (budget)    -- node {\midarrow} (anch);
\draw [connection]  (anch)    -- node {\midarrow} (lstm-west);
\draw [connection]  (lstm-east)    -- node {\midarrow} (lin2-west);
\draw [connection]  (lin2-east)    -- node {\midarrow} (output-west);

% \draw [connection]  (acts-east)      -- node {\midarrow} (acfc-west);
%\draw [rectangle connector, draw=black,dashed]  (output-east)  to (anch);

% \draw [rectangle connector=1cm,
% draw=black,dashed]  (output-east)  to %node[anchor=south, text=black, yshift = 7, xshift=20] {$a_{t+1}$}
% (act_next);

% \path [->, draw=black,dashed]  (act_next)  -| (acts-south);

%act_next

% \path[->,-{Stealth[scale=1.5]}] (lstm-north) edge [loop above,draw=blue,dashed] node {$h_t$} (lstm-north);

%
%  \path (output-east) -- (lstm-east) coordinate[pos=1] (cr1-west) ;
% \draw (d16-near)++(0,0,-1+\skipshift) coordinate (d16h);
% \draw [connection]  (after4)    -- node {\midarrow} ++(0,0,3+\skipshift) -- node {\midarrow} (score8-west);
% \draw [connection]  (score8-east) -- node{\midarrow} (d16h) -- node{\midarrow}(d16-near);
% %
% \path (cr3-east) -- (p3-west) coordinate[pos=0.4] (after3) ;
% \draw (d8-near)++(0,0,4+\skipshift) coordinate (d8h);
% \draw [connection]  (after3)    -- node {\midarrow} ++(0,0,8+\skipshift) -- node {\midarrow} (score4-west);
% \draw [connection]  (score4-east) -- node{\midarrow} (d8h) -- node{\midarrow}(d8-near);
% %
% \path (cr2-east) -- (p2-west) coordinate[pos=0.4] (after2) ;
% \draw (d4-near)++(0,0,9+\skipshift) coordinate (d4h);
% \draw [connection]  (after2)    -- node {\midarrow} ++(0,0,13+\skipshift) -- node {\midarrow} (score2-west);
% \draw [connection]  (score2-east) -- node{\midarrow} (d4h) -- node{\midarrow}(d4-near);
% %
% \path (cr1-east) -- (p1-west) coordinate[pos=0.4] (after1) ;
% \draw (d2-near)++(0,0,18+\skipshift) coordinate (d2h);
% \draw [connection]  (after1)    -- node {\midarrow} ++(0,0,22+\skipshift) -- node {\midarrow} (score-west);
% \draw [connection]  (score-east) -- node{\midarrow} (d2h) -- node{\midarrow}(d2-near);

% \draw [connection]  (d2-east)    -- node {\midarrow} (output-west);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{tikzpicture}


==> source files/illust.tex <==



\begin{tikzpicture}[scale=0.7]
\draw[step=1cm,gray,very thin] (-2,-2) grid (6,6);
\filldraw[fill=black!40!white, draw=black] (0,0) rectangle (2,2);
\filldraw[fill=black!40!white, draw=black] (2,5) rectangle (6,6);

\filldraw[fill=green!70!white, draw=black] (-2,-2) rectangle (-1,-1);
\node [quadcopter top,fill=white,draw=black,minimum width=1cm,rotate=20,scale=0.5] at (-1.5,-1.5) {}; 
\filldraw[fill=green!70!white, draw=black] (4,1) rectangle (5,2);
\filldraw[fill=green!70!white, draw=black] (1,5) rectangle (2,6);

\draw[red,thick,dashed,->] (4.5,1.5) -- (4.5,2.5);
\draw[red,thick,dashed,->] (4.5,1.5) -- (4.5,0.5);
%\draw[red,thick,dashed,->] (4.5,1.5) -- (3.5,2.5);
\draw[red,thick,dashed,->] (4.5,1.5) -- (3.5,1.5);
%\draw[red,thick,dashed,->] (4.5,1.5) -- (3.5,0.5);
%\draw[red,thick,dashed,->] (4.5,1.5) -- (5.5,2.5);
\draw[red,thick,dashed,->] (4.5,1.5) -- (5.5,1.5);
%\draw[red,thick,dashed,->] (4.5,1.5) -- (5.5,0.5);
\end{tikzpicture}

==> source files/init.tex <==
%\ProvidesPackage{init}
\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolor{rgb:blue,4;red,1;green,4;black,3}
\newcommand{\midarrow}{\tikz \draw[-Stealth,line width =0.8mm,draw=\edgecolor] (-0.3,0) -- ++(0.3,0);}

\usepackage{Ball}
\usepackage{Box}
\usepackage{RightBandedBox}



==> source files/statespace_illust.tex <==
%Author: Marco Miani
%SWAN (developed by SWAN group, TU Delft, The Netherlands) is a wave spectral numerical model.
%For Simlating WAves Nearshore, it is necessary to define spatial grids of
%physical dominant factors (wind friction, dissipation) as well as define a COMPUTATIONAL
%grid on which the model performs its (spectral) calculations: budgeting energy spectra over
%each cell of the (computational) grid. Grids might have different spatial resolution and extension.


\usetikzlibrary{positioning}



\begin{tikzpicture}[scale=.45,every node/.style={minimum size=1cm},on grid]
		
    %slanting: production of a set of n 'laminae' to be piled up. N=number of grids.
    \begin{scope}[
    	yshift=-166,every node/.append style={
    	yslant=0.5,xslant=-1},yslant=0.5,xslant=-1]
    	\fill[white,fill opacity=0.9] (0,0) rectangle (8,8);
        \draw[gray,very thin] (0,0) grid (8,8); %defining grids
        %\draw[step=1mm, red!50,thin] (3,1) grid (4,2);  %Nested Grid
        \draw[black,very thick] (0,0) rectangle (8,8);%marking borders
        \fill[orange,fill opacity=.5] (0.05,0.05) rectangle (1,1);
        \node at (0.5,0.5) {$1$};
        \fill[orange,fill opacity=.5] (0,2) rectangle (1,1);
        \node at (0.5,1.5) {$1$};
        \fill[orange,fill opacity=.5] (2,0) rectangle (1,1);
        \node at (1.5,0.5) {$1$};
    \end{scope}
    
    \begin{scope}[
            yshift=-83,every node/.append style={
            yslant=0.5,xslant=-1},yslant=0.5,xslant=-1
            ]
        % opacity to prevent graphical interference
        \fill[white,fill opacity=0.9] (0,0) rectangle (8,8);
        \draw[gray,very thin] (0,0) grid (8,8); %defining grids
        %\draw[step=1mm, red!50,thin] (3,1) grid (4,2);  %Nested Grid
        \draw[black,very thick] (0,0) rectangle (8,8);%marking borders
        \fill[red,fill opacity=.5] (2,2) rectangle (1,1);
        \node at (1.5,1.5) {$1$};
        %Idem as above, for the n-th grid:
    \end{scope}
    	
    \begin{scope}[
    	yshift=0,every node/.append style={
    	    yslant=0.5,xslant=-1},yslant=0.5,xslant=-1
    	             ]
        \fill[white,fill opacity=.9] (0,0) rectangle (8,8);
        \draw[black,very thick] (0,0) rectangle (8,8);
        \draw[gray,very thin] (0,0) grid (8,8);
        \fill[green,fill opacity=.5] (0.05,0.05) rectangle (1,1);
        \fill[green,fill opacity=.5] (6,3) rectangle (7,4);
        \fill[green,fill opacity=.5] (3,7) rectangle (4,8);
        \node at (0.5,0.5) {$1$};
        \node at (6.5,3.5) {$1$};
        \node at (3.5,7.5) {$1$};
    \end{scope}
    
       \begin{scope}[
    	yshift=83,every node/.append style={
    	    yslant=0.5,xslant=-1},yslant=0.5,xslant=-1
    	             ]
        \fill[white,fill opacity=.6] (0,0) rectangle (8,8);
        \draw[black,very thick] (0,0) rectangle (8,8);
        \draw[black] (0,0) grid (8,8);
        \fill[fill=black!40!white, fill opacity=.5] (2,2) rectangle (4,4);
        \fill[fill=black!40!white, fill opacity=.5] (4,7) rectangle (8,8);
        \node at (2.5,2.5) {$1$};
        \node at (3.5,2.5) {$1$};
        \node at (3.5,3.5) {$1$};
        \node at (2.5,3.5) {$1$};
        
        \node at (4.5,7.5) {$1$};
        \node at (5.5,7.5) {$1$};
        \node at (6.5,7.5) {$1$};
        \node at (7.5,7.5) {$1$};
    \end{scope}
    
    
    
    	
    % \begin{scope}[
    % 	yshift=170,every node/.append style={
    % 	    yslant=0.5,xslant=-1},yslant=0.5,xslant=-1
    % 	  ]
    %     \fill[white,fill opacity=0.6] (0,0) rectangle (5,5);
    %     \draw[step=10mm, black] (2,2) grid (5,5);
    %     \draw[step=2mm, green] (2,2) grid (3,3);
    %     \draw[black,very thick] (2,2) rectangle (5,5);
    %     \draw[black,dashed] (0,0) rectangle (5,5);
    % \end{scope}
    	
    % \begin{scope}[
    %     yshift=-170,every node/.append style={
    %     yslant=0.5,xslant=-1},yslant=0.5,xslant=-1
    %               ]
    %     %marking border
    %     \draw[black,very thick] (0,0) rectangle (5,5);

    %   	%drawing corners (P1,P2, P3): only 3 points needed to define a plane.
    %     \draw [fill=lime](0,0) circle (.1) ;
    %     \draw [fill=lime](0,5) circle (.1);
    %     \draw [fill=lime](5,0) circle (.1);
    %     \draw [fill=lime](5,5) circle (.1);

    %     %drawing bathymetric hypotetic countours on the bottom grid:    	
    %     \draw [ultra thick](0,1) parabola bend (2,2) (5,1)  ;
    %     \draw [dashed] (0,1.5) parabola bend (2.5,2.5) (5,1.5) ;
    %     \draw [dashed] (0,2) parabola bend (2.7,2.7) (5,2)  ;
    %     \draw [dashed] (0,2.5) parabola bend (3.5,3.5) (5,2.5)  ;
    %     \draw [dashed] (0,3.5)  parabola bend (2.75,4.5) (5,3.5);
    %     \draw [dashed] (0,4)  parabola bend (2.75,4.8) (5,4);
    %     \draw [dashed] (0,3)  parabola bend (2.75,3.8) (5,3);
    %     \draw[-latex,thick](2.8,1)node[right]{$\mathsf{Shoreline}$}
    %              to[out=180,in=270] (2,1.99);
    % \end{scope} %end of drawing grids

    %putting arrows and labels:
    \draw[-latex,thick,gray](6.6,5)node[right]{Obstacles}
        to[out=180,in=90] (4.1,5);
        
    \draw[-latex,thick,green] (4.2,2) node[right]{Charging stations}
         to[out=180,in=90] (2,2);

    \draw[-latex,thick,red](4,-.3)node[right]{Current location}
        to[out=180,in=90] (1.9,-1);
        
        \draw[-latex,thick,orange](3.9,-3)node[right]{Past locations}
        to[out=180,in=90] (2,-3.5);
        
    

    % \draw[-latex,thick](5.9,5)node[right]{$\mathsf{Wind\ G.}$}
    %     to[out=180,in=90] (3.6,5);

    % \draw[-latex,thick](5.9,8.4)node[right]{$\mathsf{Friction\ G.}$}
    %     to[out=180,in=90] (3.2,8);

    % \draw[-latex,thick,red](5.3,-4.2)node[right]{$\mathsf{G. Cell}$}
    %     to[out=180,in=90] (0,-2.5);

    % \draw[-latex,thick,red](4.3,-1.9)node[right]{$\mathsf{Nested\ G.}$}
    %     to[out=180,in=90] (2,-.5);

    % \draw[-latex,thick](4,-6)node[right]{$\mathsf{Batymetry}$}
    %     to[out=180,in=90] (2,-5);	
    % %drawing points on grid's conrners.
    % \fill[black,font=\footnotesize]
    %     (-5,-4.3) node [above] {$P_{1}$}
    %     (-.3,-5.6) node [below] {$P_{2}$}
    %     (5.5,-4) node [above] {$P_{3}$};	
\end{tikzpicture}

